Learning in the Repeated Secretary Problem

In the classical secretary problem, one attempts to find the maximum of an unknown and unlearnable distribution through sequential search. In many real-world searches, however, distributions are not entirely unknown and can be learned through experience. To investigate learning in such a repeated secretary problem we conduct a large-scale behavioral experiment in which people search repeatedly from fixed distributions. In contrast to prior investigations that find no evidence for learning in the classical scenario, in the repeated setting we observe substantial learning resulting in near-optimal stopping behavior. We conduct a Bayesian comparison of multiple behavioral models which shows that participants' behavior is best described by a class of threshold-based models that contains the theoretically optimal strategy. Fitting such a threshold-based model to data reveals players' estimated thresholds to be surprisingly close to the optimal thresholds after only a small number of games.

==> treat_results.tex <==
\subsection{Treatment Effects on Learning}

Next we turn to how learning was affected by the various
treatments. Comparing the left column of Figure \ref{fig:win_rate6} to the
right column shows that the the win rates of the 15 box treatments were
lower than the win rates of the 7 box treatments.  Recall the optimal win
rates for the 15 box treatment was .599 and the optimal win rate of the 7
box treatment was .622 (from Table \ref{tbl:1}).  Figure
\ref{fig:win_rate6} shows a much bigger difference in human behavior than
this small theoretical difference of .023 might predict. 
This might be explained by the types of errors made
in the 15 box treatments.  Figure \ref{fig:prob_win} makes it easy to see
that in the 15 box treatment people 
were much more likely to stop before the maximum box appeared (blue curves) whereas
stopping before or after the maximum box appeared was about equally likely
for the 7 box case.  On average 4.35 boxes were opened in the 7 box
treatments (62.1\% of 7), whereas 8.37 boxes were opened in the 15 box treatment
(55.8\% of 15). It appears in the 15 box condition, that people were a little too eager to stop, or a little 
too impatient. The effort involved in clicking the
mouse could be one explanation for this: as the number of boxes increases
it takes more work to open a theoretically appropriate number of boxes. 

\begin{figure}[t]
\centering
\includegraphics[width=0.75\textwidth]{../Database/final_figs/play_num_v_win_rate_noreferrals_errors_6panel.pdf}
\caption{Rates of winning (red lines), stopping too soon (blue lines) and stopping too late (green lines) for varying levels of experience by treatment condition.}
\label{fig:win_rate6}
\end{figure}

Recall the values shown to the users were drawn from the three
distributions shown in Figure \ref{fig:drawn_dists}.  The rows in Figure
\ref{fig:win_rate6} correspond to each of these three distributions.  The
right skewed distribution has the lowest win rates and the highest error
rates than any of the other three distributions.  This might sound puzzling
at first glance because the actual values drawn from the distributions are
irrelevant to succeeding at this game.  All one needs is the percentiles of
the values.  Recall that in the ``high'' distribution, boxes values were
strongly positively skewed towards the maximum of 100 million. Among 15
boxes, the average difference between the maximum value and the next
highest is relatively small at only about 80,000 dollars.  Thus it might
have been cognitively more difficult for participants to
discover a critical value in such a small range.  It also might have been more
visually difficult for participants to check if a number crossed a given
critical value given the number of digits acting as a type of visual noise.

Despite having no logical bearing on how much someone should search,
the randomly-assigned distributions had a strong effect on search depth.
Figure \ref{fig:search_depth6} shows that, relative to the uniform distribution,
people opened more boxes in the low distribution and fewer in the high distribution. 
This effect is visible in the error rates in Figure \ref{fig:win_rate6}, which shows
that rates of stopping too soon are elevated in the high distribution conditions. 
Further research is needed to determine the cause of the early stopping, but it
could have to do with values in the high condition appearing tantalizingly
close to 100 million and thus too good to pass up. 

\begin{figure}[t]
\centering
\includegraphics[width=0.75\textwidth]{../Database/final_figs/search_noreferrals_depth_6cond.pdf}
\caption{Search depth for players by randomly assigned distribution. Error
          bars indicate $\pm 1$ standard error}
\label{fig:search_depth6}
\end{figure}

%% SS to DG:  Here I'm saying the participants learned more quickly in the
%% 15 box game but above we say they had lower win rates.  That doesn't
%% make sense.  Should we cut this plot?
%%   skew_factor num_boxes mean_boxes_opened mean_boxes_opend_se
%% 1           1         7          4.439504          0.02339391
%% 2           1        15          8.814391          0.06457514
%% 3           2         7          4.375600          0.02627313
%% 4           2        15          8.232962          0.06694627
%% 5           3         7          4.199752          0.02708407
%% 6           3        15          8.006180          0.07513678
%%   skew_factor num_boxes num_played_avg num_played_se
%% 1           1         7      10.253880     1.1761985
%% 2           1        15       7.111745     0.3863313
%% 3           2         7       8.952941     0.7453443
%% 4           2        15       6.681111     0.3148676
%% 5           3         7       8.492571     0.5285379
%% 6           3        15       6.330882     0.3396461

